FO and MSO Model Checking on Temporal Graphs

Algorithmic meta-theorems provide an important tool for showing tractability of graph problems on graph classes defined by structural restrictions. While such results are well established for static graphs, corresponding frameworks for temporal graphs are comparatively limited. In this work, we revisit past applications of logical meta-theorems to temporal graphs and develop an extended unifying logical framework. Our first contribution is the introduction of logical encodings for the parameters vertex-interval-membership (VIM) width and tree-interval-membership (TIM) width, parameters which capture the signature of vertex and component activity over time. Building on this, we extend existing monadic second-order (MSO) meta-theorems for bounded lifetime and temporal degree to the parameters VIM and TIM width, and establish novel first-order (FO) meta-theorems for all four parameters. Finally, we signpost a modular lexicon of reusable FO and MSO formulas for a broad range of temporal graph problems, and give an example. This lexicon allows new problems to be expressed compositionally and directly yields fixed-parameter tractability results across the four parameters we consider.

==> _macros-mso-list.tex <==

\definecolor{RED}{rgb}{0.82, 0.1, 0.26}

% ======= Minimal MSO formula catalog (LIPIcs-friendly) =======
\makeatletter
% Counter MSO formulas within subsections
\newcounter{msoformula}[subsection]
\renewcommand{\themsoformula}{\thesubsection.\arabic{msoformula}}

%======================= Current category (shown in the lexicon); set manually
\newcommand{\MSO@CurrentCategory}{General}
\newcommand{\MSOSetCategory}[1]{\gdef\MSO@CurrentCategory{#1}}

%======================= Store: titles, a simple list body, and a lexicon body
\newcommand{\MSO@settitle}[2]{\expandafter\gdef\csname mso@title@#1\endcsname{#2}}
\newcommand{\MSO@gettitle}[1]{\@ifundefined{mso@title@#1}{#1}{\csname mso@title@#1\endcsname}}
\newcommand{\MSO@ListBody}{}       % one-line per formula for the “List”
\newcommand{\MSO@LexiconBody}{}    % rows for the lexicon table

\newlength{\msoskip}
\setlength{\msoskip}{\topsep} % or try 0.6\baselineskip to taste


% ---- (A) metadata storage: logic + source + used-in list ----
\newcommand{\MSO@setlogic}[2]{\expandafter\gdef\csname mso@logic@#1\endcsname{#2}}
\newcommand{\MSO@getlogic}[1]{\@ifundefined{mso@logic@#1}{MSO}{\csname mso@logic@#1\endcsname}}

\newcommand{\MSO@setsource}[2]{\expandafter\gdef\csname mso@source@#1\endcsname{#2}}
\newcommand{\MSO@getsource}[1]{\@ifundefined{mso@source@#1}{novel}{\csname mso@source@#1\endcsname}}

% used-in list stored as comma-separated tokens in \mso@usedin@<key>
\newcommand{\MSO@usedin@init}[1]{%
  \@ifundefined{mso@usedin@#1}{\expandafter\gdef\csname mso@usedin@#1\endcsname{}}{}%
}
\newcommand{\MSO@getusedin}[1]{%
  \@ifundefined{mso@usedin@#1}{}{%
    \csname mso@usedin@#1\endcsname
  }%
}

% add "source formula key" to "target formula key"'s used-in list (avoid duplicates)
\newcommand{\MSO@recorduse}[2]{% target=#1, source=#2
  \MSO@usedin@init{#1}%
  \edef\MSO@tmp{\csname mso@usedin@#1\endcsname}%
  \edef\MSO@add{#2}%
  \ifx\MSO@add\@empty\else
    \ifinlist{\MSO@add}{\MSO@tmp}{}{%
      \ifx\MSO@tmp\@empty
        \expandafter\gdef\csname mso@usedin@#1\endcsname{#2}%
      \else
        \expandafter\gdef\csname mso@usedin@#1\endcsname{\MSO@tmp,#2}%
      \fi
    }%
  \fi
}

% current formula key (while typesetting an MSOFormula body)
\newcommand{\MSO@CurrentKey}{} % empty when not inside a formula

% pretty printer for used-in list (prints hyperlinks to formulas)
    \newcommand{\MSO@printusedin}[1]{%
      \begingroup
      \edef\MSO@tmp{\MSO@getusedin{#1}}%
      \ifx\MSO@tmp\@empty
        none%
      \else
        \def\do##1{\mso{##1}\,}%
        \expandafter\docsvlist\expandafter{\MSO@tmp}%
      \fi
      \endgroup
    }


\newcommand{\PrintMSOWhereUsed}[1]{%
  \par\noindent\emph{Used in:}~\MSO@printusedin{#1}\par
}


%=====================================================================================================
%=====================================================
%=====================================================
%================ MAIN MACRO: \MSOFormula{key}{Title}{Purpose}{Free vars}{Parameters}{Length}{Body}{Logic}{Reference} =============================
% \MSOFormula{key}{Title}{Purpose}{Free vars}{Parameters}{Length}{Body}[Logic][Source]
%=====================================================
%=====================================================
\newcommand{\MSOFormula}[9]{%{m m m m m m m O{MSO} O{novel}}{%
    \refstepcounter{msoformula}%
    \vspace{0.5em}
    \MSO@settitle{#1}{#2}%
    \MSO@setlogic{#1}{#8}%
    \MSO@setsource{#1}{#9}%
    \MSO@usedin@init{#1}%
    \label{mso:#1}%

    % mark current formula key so \msovarphi can record "where used"
    % \gdef\MSO@CurrentKey{#1}%

    \noindent\textbf{#8 Formula \themsoformula\quad #2}\par\vspace{0.05em}\noindent
    \emph{Purpose:}~#3\par\vspace{0.05em}\noindent
    % \begin{tabular}{p{0.1\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.5\linewidth}@{}}
    % \emph{Logic:}      & #8  & \emph{Source:}   & #9 \\
    % \emph{Length:}     & #6  & \emph{Encodings:} & #5 
    % \end{tabular}
    {\renewcommand{\arraystretch}{0.95}%
    \begin{tabular}{@{}p{0.07\linewidth}p{0.11\linewidth}p{0.08\linewidth}p{0.13\linewidth}p{0.12\linewidth}p{0.30\linewidth}@{}}
    \emph{Logic:}  & #8 & \emph{Length:}    & #6 & \emph{Encodings:} & #5 
    \end{tabular}}
    \[
        \begin{aligned}
            % \varphi_{\text{#1}}(#4)&:= #7
            % \varphi_{\text{#1}}&(#4)= #7
            &\varphi_{\text{#1}}(#4)= #7
        \end{aligned}
    \]

    % leave the "current formula" context
    \gdef\MSO@CurrentKey{}%
    
    % Append to the simple “List”
    \g@addto@macro\MSO@ListBody{%
      \noindent\hyperref[mso:#1]{MSO Formula \ref*{mso:#1}~(\MSO@gettitle{#1})}%
      \dotfill \pageref{mso:#1}\par
    }%

    % Append a lexicon row (extended with Logic + Source)
    \g@addto@macro\MSO@LexiconBody{%
      #2 & #3 & \MSO@CurrentCategory & \MSO@getlogic{#1} & \ref{mso:#1} & #6 & \MSO@getsource{#1}\\
    }%
}
%=====================================================
%=====================================================

%=====================================================
%================ MAIN MACRO: \MSOFormula{key}{Title}{Purpose}{Free vars}{Parameters}{Length}{Body}{Logic}{Reference} =============================
% \MSOFormula{key}{Title}{Purpose}{Free vars}{Parameters}{Length}{Body}[Logic][Source]
%=====================================================
%=====================================================
\newcommand{\MSOFormulaD}[9]{%{m m m m m m m O{MSO} O{novel}}{%
    \refstepcounter{msoformula}%
    \vspace{0.5em}
    \MSO@settitle{#1}{#2}%
    \MSO@setlogic{#1}{#8}%
    \MSO@setsource{#1}{#9}%
    \MSO@usedin@init{#1}%
    \label{mso:#1}%

    % mark current formula key so \msovarphi can record "where used"
    % \gdef\MSO@CurrentKey{#1}%

    \noindent\textbf{#8 Formula \themsoformula\quad #2}\par\noindent
    \emph{Purpose:}~#3\par\noindent
    % \begin{tabular}{p{0.1\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.5\linewidth}@{}}
    % \emph{Logic:}      & #8  & \emph{Source:}   & #9 \\
    % \emph{Length:}     & #6  & \emph{Encodings:} & #5 
    % \end{tabular}
    {\renewcommand{\arraystretch}{0.95}%
    \begin{tabular}{@{}p{0.07\linewidth}p{0.11\linewidth}p{0.08\linewidth}p{0.13\linewidth}p{0.12\linewidth}p{0.30\linewidth}@{}}
    \emph{Logic:}  & #8 & \emph{Length:}    & #6 & \emph{Encodings:} & #5 
    \end{tabular}}
    \[
        \begin{aligned}
            % \varphi_{\text{#1}}(#4)&:= #7
            % \varphi_{\text{#1}}&(#4)= #7
            &{\varphi_{\text{#1}}}_{#4} #7
        \end{aligned}
    \]

    % leave the "current formula" context
    \gdef\MSO@CurrentKey{}%
    
    % Append to the simple “List”
    \g@addto@macro\MSO@ListBody{%
      \noindent\hyperref[mso:#1]{MSO Formula \ref*{mso:#1}~(\MSO@gettitle{#1})}%
      \dotfill \pageref{mso:#1}\par
    }%

    % Append a lexicon row (extended with Logic + Source)
    \g@addto@macro\MSO@LexiconBody{%
      #2 & #3 & \MSO@CurrentCategory & \MSO@getlogic{#1} & \ref{mso:#1} & #6 & \MSO@getsource{#1}\\
    }%
}
%=====================================================

%=====================================================================================================

% Compact referencing in text (if you ever need it):
\newcommand{\mso}[1]{MSO Formula~\ref{mso:#1}~(\MSO@gettitle{#1})}

%================== Print a simple, hyperlinked List of MSO Formulas===============
\newcommand{\PrintMSOList}{%
  \section*{List of MSO Formulas}%
  \begingroup
    \MSO@ListBody
  \endgroup
}

%================== Print a LEXICON TABLE ===========================
        \newcommand{\PrintMSOLexicon}{%
            \section*{MSO Formula Lexicon}
            \begingroup
            \setlength{\tabcolsep}{6pt}\renewcommand{\arraystretch}{1.1}%
            \begin{tabular}{@{}p{0.20\linewidth}p{0.30\linewidth}p{0.16\linewidth}p{0.06\linewidth}p{0.04\linewidth}p{0.08\linewidth}p{0.12\linewidth}@{}}
                \textbf{Name} & \textbf{What it expresses} & \textbf{Category} &
                \textbf{Logic} & \textbf{Ref.} & \textbf{Length} \\\hline
                \MSO@LexiconBody
            \end{tabular}
        %     \begin{tabular}{@{}p{0.22\linewidth}p{0.34\linewidth}p{0.2\linewidth}p{0.04\linewidth}p{0.08\linewidth}@{}}
        %         \textbf{Name} & \textbf{What it expresses} &
        %         \textbf{Category} & \textbf{Ref.} & \textbf{Length}\\\hline
        %         \MSO@LexiconBody
        %     \end{tabular}
            \endgroup
        }
%===================================================================

%================ MSO FORMULAS Usage ============================
% \msovarphi{key}           ->  \varphi_{\text{key}}   (hyperlinked to mso:key)
% \msovarphi*{key}          ->  same, but no hyperlink (safe in headings)
% \msovarphi{key}[args]     ->  \varphi_{\text{key}}(args)
        \NewDocumentCommand{\msovarphi}{s m o}{%
          \ensuremath{%
            \IfBooleanTF{#1}{%
              \varphi_{\text{#2}}%
            }{%
              \hyperref[mso:#2]{\varphi_{\text{#2}}}%
            }%
            \IfValueT{#3}{\!\left(#3\right)}%
          }%
        }

% \RenewDocumentCommand{\msovarphi}{s m o}{%
%   \ifx\MSO@CurrentKey\@empty\else
%     \MSO@recorduse{#2}{\MSO@CurrentKey}%
%   \fi
%   \ensuremath{%
%     \IfBooleanTF{#1}{%
%       \varphi_{\text{#2}}%
%     }{%
%       \hyperref[mso:#2]{\varphi_{\text{#2}}}%
%     }%
%     \IfValueT{#3}{\!\left(#3\right)}%
%   }%
% }
\RenewDocumentCommand{\msovarphi}{s m o}{%
  \ensuremath{%
    \IfBooleanTF{#1}{%
      \varphi_{\text{#2}}%
    }{%
      \hyperref[mso:\MSO@resolvetarget{#2}]{\varphi_{\text{#2}}}%
    }%
    \IfValueT{#3}{\!\left(#3\right)}%
  }%
}


% Convenience alias if you prefer mandatory args:
% \msovarphiof{key}{args}
\NewDocumentCommand{\msovarphiof}{m m}{%
  \ensuremath{\hyperref[mso:#1]{\varphi_{\text{#1}}}\!\left(#2\right)}%
}



%======== AN ALIAS for deg=k used with deg=1, ....$ ========
% Define an alias: key -> targetkey (hyperlink target)
\newcommand{\msoalias}[2]{%
  \expandafter\gdef\csname mso@alias@#1\endcsname{#2}%
}

% Resolve a key to its hyperlink target (defaults to itself)
\newcommand{\MSO@resolvetarget}[1]{%
  \@ifundefined{mso@alias@#1}{#1}{\csname mso@alias@#1\endcsname}%
}



\makeatother





